SeafloorAI: A Large-scale Vision-Language Dataset for Seafloor Geological Survey

A major obstacle to the advancements of machine learning models in marine science, particularly in sonar imagery analysis, is the scarcity of AI-ready datasets. While there have been efforts to make AI-ready sonar image dataset publicly available, they suffer from limitations in terms of environment setting and scale. To bridge this gap, we introduce SeafloorAI, the first extensive AI-ready datasets for seafloor mapping across 5 geological layers that is curated in collaboration with marine scientists. We further extend the dataset to SeafloorGenAI by incorporating the language component in order to facilitate the development of both vision- and language-capable machine learning models for sonar imagery. The dataset consists of 62 geo-distributed data surveys spanning 17,300 square kilometers, with 696K sonar images, 827K annotated segmentation masks, 696K detailed language descriptions and approximately 7M question-answer pairs. By making our data processing source code publicly available, we aim to engage the marine science community to enrich the data pool and inspire the machine learning community to develop more robust models. This collaborative approach will enhance the capabilities and applications of our datasets within both fields.

==> Styles/sections/3_tasks.tex <==
\section{Task Formulation}
We present two machine learning tasks: (1) seafloor mapping and (2) target object detection.

\subsection{Pre-task: Self-supervised Learning}
\noindent\textbf{Task formulation.}

\noindent\textbf{Experiment setup.}

\subsection{Task A: Seafloor Mapping}
\noindent\textbf{Task formulation.} 
We propose to map different GIS layers, including \texttt{Fault}, \texttt{Fold}, \texttt{Sediment}, \texttt{Physiographic Zone}, and \texttt{Habitat}, from acoustic remote sensing data (\texttt{Backscatter} and \texttt{Bathymetry}).
The primary task we are addressing is semantic segmentation, which involves categorizing each pixel in an image into one of several classes based on the data provided by these layers. 
For the \texttt{Fault} and \texttt{Fold} layers, this involves a binary segmentation task, distinguishing only between the presence or absence of these features. 
For the \texttt{Sediment}, \texttt{Physiographic Zone}, and \texttt{Habitat} layers, we specify a multi-class segmentation task, which requires assigning each pixel to one of several predefined categories. 
This structure is designed to facilitate detailed environmental seafloor analysis and interpretation. 

\noindent\textbf{Experiment setup.}

\noindent\textbf{Results.}

\subsection{Task B: Target Object Detection}
\noindent\textbf{Task formulation.}

\noindent\textbf{Experiment setup.}

\noindent\textbf{Results.}


==> Styles/sections/X_how_data_collect.tex <==
\section{A Brief Overview on Multibeam Data Collection}
% Figure + explanation of how multibeam backscatter and bathymetry data is collected.
% https://www.ga.gov.au/scientific-topics/marine/survey-techniques/backscatter

Multibeam echosounder mounted on a survey vessel collects backscatter and bathymetry at the ssame time. Backscatter intensity reflects the seafloor hardness, and bathymetry measures the ocean depth. 

During data collection, multibeam echosounders send out multiple sound waves that bounce off the sea floor and return to the ship. These sound waves are emitted as acoustic pulses. From each pulse, a co-located bathymetry and backscatter measurement is collected. Each acoustic pulse propagates from the vessel in a line of beams from left to right, fanning out under the vessel; this is known as the beam pattern. The beam pattern is wide across-track, which means it covers the area immediately under the vessel, and on either side of the vessel, and narrow along-track, which means it does not cover the area in front or behind the vessel.

The delay between sending the signal from the transmit arrays and receiving the acoustic returns provides a measurement of ocean depth, or bathymetry data. The strength of the return signal provides an indication of how hard the sea floor is, or backscatter data.
